Demystifying the Performance of Data Transfers in High-Performance Research Networks

High-speed research networks are built to meet the ever-increasing needs of data-intensive distributed workflows. However, data transfers in these networks often fail to attain the promised transfer rates for several reasons, including I/O and network interference, server misconfigurations, and network anomalies. Although understanding the root causes of performance issues is critical to mitigating them and increasing the utilization of expensive network infrastructures, there is currently no available mechanism to monitor data transfers in these networks. In this paper, we present a scalable, end-to-end monitoring framework to gather and store key performance metrics for file transfers to shed light on the performance of transfers. The evaluation results show that the proposed framework can monitor up to 400 transfers per host and more than 40, 000 transfers in total while collecting performance statistics at one-second precision. We also introduce a heuristic method to automatically process the gathered performance metrics and identify the root causes of performance anomalies with an F-score of 87 - 98%.

==> 4_d_real_world_application.tex <==

\begin{figure}
\begin{center}
% \vspace{-5mm}
\includegraphics[keepaspectratio=true,angle=0,width=0.48\textwidth] {figures/new_evaluation_results/Real_world_montage.pdf}
\vspace{-3mm}
\caption{Impact of I/O congestion caused by real-world HPC application on the performance of file transfer.}
\label{fig:montage_app_evaluation}
\end{center}
%\hspace{-20mm}
\vspace{-6mm}
\end{figure}

We next present the effectiveness of the proposed monitoring framework in detecting the root cause of performance problems when a transfer application is competing with an HPC application for I/O resources. To do so, we execute the Montage~\cite{jacob2009montage} application on the sender side in Testbed-1 while the transfer process is going on. Montage transforms input images from flexible image transport system (FITS) format to custom mosaics of the sky. It is characterized as a data-intensive application due to issuing a significant volume of write operations. %In this experiment, we build a 1.5 deg x 1.5 deg mosaic of 91 2MASS K-band images centered on M17. We first generate a mosaic without a background correction. This phase consists of six stages. Next, to smooth out the background levels between overlapping images, in phase 2, we perform seven more stages for background corrections leading to 13 stages to create the final mosaic image. 
We observe that each Montage application issues around $3$GiB write I/O during its execution. Thus, we execute five instances of the Montage application and store their output on the same OST that the transfer process is using to write files. As a result, we expect that it will trigger write congestion on the OST. 

Figure~\ref{fig:montage_app_evaluation} shows the effect of running Montage applications along with the transfer process on the throughput of the transfer. While the throughput of the transfer is around $3.7$ Gbps at the beginning, it drops to around $2$ Gbps as Montage jobs start writing to the file system at around $35s$. Similarly, Montage applications issue more write operations between $56s-82s$ and $108s-158$, which causes transfer throughout to drop to $2-2.5$ Gbps due to write congestion on the OST. 
We next used the proposed heuristic model. Blue circles mark the times the model predicts I/O congestion when performance metrics for the transfer are fetched from the Elastic Search and given to the model in real time. Overall, out of $114$ intervals during which Montage applications issued write operations, the model successfully identified $100$ as write congestion. Thus it is fair to say that the heuristic model is quite effective at processing real-time performance metrics as they are being captured to identify performance issues in a timely way. 
% We next tested the performance of Random Forest model trained using the data collected in Testbed-3 with five labels. Blue circles marks the times that the Random Forest model predicts sender-side I/O congestion when performance metrics for the transfer are fetched from the Elastic Search and given to the model in real-time. Overall, out of $114$ intervals during which Montage applications issued write operations, the model successfully identified $100$ as write congestion. Consequently, machine learning models are quite effective at processing real-time performance metrics as they are being captured to identify the performance issues in a timely way. 





==> old_docs/evaluation.tex <==
\begin{figure}
%\vspace {-4mm}
\begin{centering}
\includegraphics[keepaspectratio=true,angle=0,width=0.35\textwidth]{figures/size_vs_score.pdf}
% \vspace{-3mm}
\caption{Performance comparison of Decision Tree models with respect to training sample size} 
\label{fig:size_vs_score}
% \vspace {-3mm}
\end{centering}
\end{figure}


\begin{table}
\renewcommand{\arraystretch}{1.5}
\begin{centering}
\caption{Cross-Validation Results}
\label{tab:eval_cross_validation}
\resizebox{.45\textwidth}{!}{
\begin{tabular}{|p{4cm} | p{2cm}|p{2cm} | p{2cm}|}
\hline
{\bf Classification Model } & {\bf Testbed \#1}   & {\bf Testbed \#2} & {\bf Testbed \#3} \\
\hline
\textbf{Support Vector Classifier} & 95.28 $\pm$ 2.92 & 96.57 $\pm$ 2.19 & 97.33 $\pm$ 1.45 \\
\hline
\textbf{Neural Network} & 97.25 $\pm$ 1.23 & 98.32 $\pm$ 0.79 & 97.86 $\pm$ 1.46 \\
\hline
\textbf{Decision Tree} & 96.84 $\pm$ 1.65 & 97.09 $\pm$ 1.07 & 97.13 $\pm$ 2.39 \\
\hline
\textbf{XGBoost} & 97.11 $\pm$ 1.79 & 98.09 $\pm$ 1.1 & 98.6 $\pm$ 1.19 \\
\hline
\textbf{Random Forest} & 97.37 $\pm$ 1.33 & 97.7 $\pm$ 1.5 & 97.92 $\pm$ 1.75 \\
\hline
\end{tabular}}
\end{centering}
% \vspace{-4mm}
\end{table}


% The neural network ran for 100 epochs with a batch size of 270. Figure~\ref{fig:nn-training} shows the accuracy and loss rate of the model during the training phase. It shows that the model can achieve 93\% accuracy rate and 0.3\% loss rate after 100 epochs.

% \begin{figure}[t]
% \begin{center}
% \vspace{-5mm}
% %\hspace{-4mm}
% \subfigure[Accuracy]{
% \includegraphics[keepaspectratio=true,angle=0,width=55mm]{figures/Images/acc3.png}
% \label{fig:accuracy}}
% \hspace{-8mm}
% \subfigure[Loss Rate]{
% \includegraphics[keepaspectratio=true,angle=0,width=55mm] {figures/Images/loss3.png}
% \label{fig:loss}}
% \vspace{-2mm}
% \caption{Accuracy and loss rate of Neural Network model during the training phase.}
% \label{fig:nn-training}
% \end{center}
% %\hspace{-20mm}
% \vspace{-8mm}
% \end{figure}

% While the model accuracy is limited to 93\% when it is tested with 30 different labels (10 anomalies with ~3 severity level for each anomaly), its performance increases to 96\% when the three different severity levels are grouped into same category as shown in Fig~\ref{fig:nn-confusion}. For example, we reproduced three different packet loss anomalies by injecting 0.1\%, 0.5\%, and 1\% losses and model performance improved slightly when these three anomaly types are marked with the same ``packet loss'' label. Similarly, the model performance improved to 99.96\% when only four labels are used as \emph{normal, server, network, and file system}. This high level categorization can be used to develop an hierarchical model where higher level predictions can be used to route the performance issues to the right the group in large organizations to facilitate ticket categorization.

% \begin{figure}[t]
% \begin{center}
% \vspace{-3mm}
% \includegraphics[keepaspectratio=true,angle=0,,width=0.75\linewidth]{figures/Images/confusion.pdf}
% \vspace{-6mm}
% \caption{Confusion matrix of the neural network model. It is able to predict the correct label with 96\% accuracy.}
% \label{fig:nn-confusion}
% \end{center}
% %\hspace{-20mm}
% \vspace{-8mm}
% \end{figure}

% %The accuracy model shows the growth of the NN with an average accuracy rate of 93\% and the loss rate was roughly 0.2. Based on figure 4, we can see that the model was able to accurately pinpoint the anomaly label with (BLANKS). With the model, we can predict with 93\% accuracy the underlying resource that was causing the anomaly and thus prove that using NN to predict underlying causes of performance anomalies is appropriate. 

% %We can accurately predict the underlying cause for the performance anomaly because we took metrics from different areas of the system and compared them as a whole system. By doing this, we are providing the neural network a large parameter set to find a pattern that may not be seen by looking at less metrics. With the neural network using the collective data, we can find a pattern in the outliers that may point to a performance anomaly that is not suspected. By looking at the data, we can see that during an anomaly that stresses the memory, the CPU will also be stressed. If we were looking at each metric separately, we would not be able to predict that the anomaly is from the memory, however, we can find the correct anomaly by looking at all of the metrics.


==> old_docs/introduction.tex <==
% %  Despite the continuous efforts to upgrade the networking infrastructure of research and education institutions to meet the large-scale data analytics needs and foster collaboration between scientists, the data transfers on these networks often perform very poorly, especially in the wide-area. The reason for the poor performance may not always be the lack of network bandwidth, but it may be due to other factors such as misconfigured servers, storage and I/O bandwidth limitations, network congestion, overloaded end systems, or other anomalies~\cite{arslan2018big,arslan2018high}.
 
% % \begin{figure}[b]
% % \begin{center}
% % \vspace{-5mm}
% % \includegraphics[keepaspectratio=true,angle=0,width=50mm] {figures/file_transfer.pdf}
% % \caption{The performance of file transfers fluctuate significantly in high-speed networks.}
% % \label{fig:throughput_variation}
% % \end{center}
% % %\hspace{-20mm}
% % \vspace{-6mm}
% % \end{figure}
 

 
 
% % the involvement of multiple end systems, dynamically changing background traffic, and the complexity of today's networking infrastructures turns it into a complicated and time-consuming process. On the other hand, it is a challenging task even for domain experts to instrument end-to-end data transfers in today's highly sophisticated networks and end systems.
 

 
%  %In addition to network bandwidth, the number of network domains is increasing rapidly as more local and regional networks emerge. As a result, wide-area data transfers travel through multiple network domains to reach their destination. Moreover, parallel file systems have been introduced to offer high-speed I/O performance and increased reliability. User data on parallel file systems are distributed among multiple storage servers, so file transfer operations need to interact with many servers to read/write files and access/update metadata information. Further, high-performance computing (HPC) clusters deploy data transfer nodes (DTNs) to support high-speed network bandwidth because it is either too expensive or impossible with current technologies to handle high-speed traffic using a single DTN. Hence, effectively monitoring and troubleshooting the performance of high-speed data transfers that are reading/writing from/to many storage servers, using multiple DTNs, and passing through many network domains is highly challenging. The shared nature of these systems exacerbates the complexity of the problem and makes troubleshooting even more difficult.
 
%  Figure~\ref{fig:throughput_variation} shows the throughput of a 7GB file transfers between the Comet and Stampede clusters when repeated for four days. The observed throughput varied drastically between 150 Mbps and 3000 Mbps. While it is possible to correlate throughput fluctuation of memory-to-memory transfers to background traffic, doing so is much more complicated for disk-to-disk transfers, because it also depends on other factors such as storage and DTN load. As many science projects require predictable and stable network performance to streamline computation and communications tasks, it is critical to identify the root causes of performance bottlenecks such that proper actions can be taken to mitigate them to utilize high-cost research networks effectively. 
 
% \begin{figure}[t]
% \begin{center}
% %\vspace{-5mm}
% \includegraphics[keepaspectratio=true,angle=0,width=85mm] {figures/end-to-end-visualization.pdf}
% \caption{End-to-end transfer performance is determined by many system components.}
% \label{fig:system-architecture}
% \end{center}
% %\hspace{-20mm}
% \vspace{-8mm}
% \end{figure}

%  %Understanding the true underlying reasons for poor transfer performance is key to mitigating them and delivering the promised transfer speeds. However, effectively monitoring and troubleshooting the performance of high-speed data transfers that are reading/writing from/to many storage servers, using multiple data transfer nodes, and passing through many network domains is highly challenging. The shared nature of these systems exacerbates the complexity of the problem and makes troubleshooting even more difficult.
 
%  A typical setup for data transfers in research networks is illustrated in Figure~\ref{fig:system-architecture}. Large-scale scientific data is generally stored in parallel file systems, causing transfers to interact with many storage servers across the cluster to read/write files and access/update metadata information. Moreover, high-performance computing clusters deploy several data transfer nodes (DTNs) to handle large numbers of concurrent transfers. Finally, transfers typically travel through many network domains before reaching their destination. Monitoring and troubleshooting the performance of high-speed data transfers that are reading/writing from/to many storage servers, using multiple DTNs, and passing through many network domains is challenging. The shared nature of these systems exacerbates the complexity and makes troubleshooting even harder.
 
%  For high-level network monitoring, PerfSonar~\cite{perfsonar} runs active measurements between research and education institutions to detect major network events such as node and link failures. It collects throughput, delay, packet re-transmission, and packet route information using measurement tools such as \textit{traceroute} and \textit{Iperf}. While it can provide useful information about network status, it can only detect persistent issues as its measurements are not continuous to avoid affecting actual science flows. Moreover, since it only collect few high-level performance metrics, it is unable to pinpoint the underlying reasons of poor transfer performance. Therefore, this project proposes online, comprehensive, and fine-grained solution to the problem of end-to-end scientific flow monitoring problem. To achieve this goal, we collect the set of key performance metrics that can capture performance of end-to-end transfers under various, commonly-observed circumstances. %{\em To the best of our knowledge, this project is making the first attempt to identify the set of metrics and their ideal resolution for accurate and online performance analysis of wide-area end-to-end data transfers in extreme-scale research networks.}

==> old_docs/model.tex <==
\begin{figure}[t]
\begin{center}
%\vspace{-5mm}
\includegraphics[keepaspectratio=true,angle=0,width=\linewidth] {figures/NN-fig.pdf}
\caption{Proposed solution to collect performance metrics in real-time to detect performance anomalies.}
\label{fig:system-architecture}
\end{center}
%\hspace{-20mm}
\vspace{-8mm}
\end{figure}

We developed an anomaly detection framework to pinpoint the root causes of performance degradation as shown in Figure~\ref{fig:system-architecture}. Unlike earlier anomaly detection studies that categorize network traffic as \textit{normal} or \textit{abnormal}, we take a step further and also find the underlying reasons for abnormalities, such as congestion in a storage server or a faulty network interface card using the real-time performance metrics.% For example, researchers introduced NetPoirot to find the root cause of traffic anomalies in datacenter networking using Random Forest~\cite{arzani2016taking}. While NetPoirot was successful in identifying the source of anomalies between client, network, or server, its accuracy degrades significantly when it attempts to determine the root cause, leaving the daunting root cause detection issue unsolved. Thus, this task will develop an anomaly detection framework to pinpoint the root causes of performance degradation by collecting key metrics in required precision.   


To train a model, we reproduced 10 common traffic anomalies with different severity levels in Chameleon Cloud network, where we created one instance in Chicago, IL and another instance in Austin, TX. The network bandwidth is 10Gbps and delay is 32ms. We collected performance metrics for file system, data transfer nodes, and TCP performance. Memory overload, disk congestion, CPU contention, packet loss, packet delay, packet duplicate, packet corrupt, packet reordering are among the anomaly types that we reproduces using the linux tools such as \texttt{tc} and \texttt{stress}. We then used \texttt{ss}, \texttt{sar}, and \texttt{iostat} utilities to collect real-time performance metrics in 100ms intervals.


Neural Network (NN) mimics human brain to detect patterns in datasets and is proved to be very effective in many areas. Therefore, we trained a NN model to process performance statistics and extract patterns between the given input metrics and anomaly types. We used a Rectified Linear Unit (ReLU) activation sequence for the hidden layers and a SoftMax activation sequence for the output layer. Activation sequences are used to signify if a neuron should be included in the next layer or not. %We used ReLU because it is fast and easy to optimize due to its similarity to linear functions while maintaining the same performance level as other activation sequences. The SoftMax activation sequence is commonly used in output layers and provides a probability of each outcome, with the target label having the highest probability. 
In addition, we used the Adam optimizer as it is useful for large data sets and is optimized for large parameter sets. We utilized Tensorflow and Keras to create build and train NN and matplotlib to provide an accuracy and loss plot. Each run used 80\% the total number of data points as the training size and 20\% as the testing size with an epoch of 100.

%\textbf{Data Collection:} We collected over 70 metrics to monitor the performance of file system, data transfer node, and network connection in 100ms intervals.
%The data that was collected included performance metrics from four different areas: disk input and output (I/O), network throughput, CPU statistics, and memory statistics. From these four categories we collected over 70 metrics. The metrics were collected using a data collection program written in python that found one data point of metrics for every 0.01 seconds. For each round we ran the collection program 31 times, once with no anomaly and 30 times with different anomalies. We created three different levels of stress over 10 different anomaly types: memory load, disk load, I/O load, CPU load, packet loss rate, packet delay, packet duplicate, packet corrupt, packet reordering, and bandwidth limit. This was to produce metrics that would more resemble real world simulations. Round one had a batch size of 300 data points and round 2-5 had 600 data points. The total amount of data points collected was 2700 and the total number of metrics collected was over 189 thousand. We then compiled all of the data into one file including the anomaly label at the beginning. We then used these metrics as the training and testing set for the neural network.
 
%The program we used to collect metrics utilized the Psutil python module for CPU, Disk I/O, and Memory metrics. As well as the Linux command iostat to find the network metric. We also used Python’s sockets module to transfer files between two systems. Files, ranging from 10 megabytes (MB) to 100 gigabytes (GB), were transferred to provide end to end file transfers later used to find the network metrics. We used the ChameleonCloud, an NSF-granted test bed, servers at the University of Texas (TACC) and the University of Chicago (UC) to provide a local-area network transfer and long-distance network transfer.
%ChameleonCloud was built on the OpenStack cloud software and utilizes over 600 nodes and 10 thousand Xion Haswell processors.[5] ChameleonCloud was used to run the collection and anomaly programs for collecting data with faster processors and hardware to simulate real-world server bottlenecks and anomalies. The anomalies shell script used the Linux commands stress-ng, stress, and tc to induce different anomalies. 

%For the NN we used the python modules Tensorflow and Keras to create the model and matplotlib to provide an accuracy and loss plot. Each run used 80\% the total number of data points as the training size and 20\% as the testing size with an epoch of 100.[6]


==> todo-list.tex <==
1- Collect data from production systems regarding the root causes of performance problems
2-Support for more file systems. The system currently supports Lustre but we need to extend it for few other file systems such as local (ext3) and beegfs
3- 
